Robust Dominant Periodicity Detection for Time Series with Missing Data

Periodicity detection is an important task in time series analysis, but still a challenging problem due to the diverse characteristics of time series data like abrupt trend change, outlier, noise, and especially block missing data. In this paper, we propose a robust and effective periodicity detection algorithm for time series with block missing data. We first design a robust trend filter to remove the interference of complicated trend patterns under missing data. Then, we propose a robust autocorrelation function (ACF) that can handle missing values and outliers effectively. We rigorously prove that the proposed robust ACF can still work well when the length of the missing block is less than $1/3$ of the period length. Last, by combining the time-frequency information, our algorithm can generate the period length accurately. The experimental results demonstrate that our algorithm outperforms existing periodicity detection algorithms on real-world time series datasets.

==> 2_related_work.tex <==
\section{Related Work}\label{sec:related}

%Periodicity detection is also referred as season length estimation~\cite{Toller2019}. 

% % Traditional two types of periodicity detecteion algorithms
% The common periodicity detection algorithms can be categorized into two groups: 1) frequency domain methods relying on periodogram after Fourier transform; 2) time domain methods relying on autocorrelation function (ACF). As periodicity detection is also referred as season length estimation~\cite{Toller2019}, we use periodicity and seasonality equivalently in this paper.
% % periodogram-based approach
% In the frequency domain methods, the periodogram measures how periodic the time series is at different frequencies. 
% % If a time series does not contain a periodic component, then the periodogram reduces to a straight line. 
% Once the periodogram is calculated, Fisher's test~\cite{fisher1929tests,wichert2004identifying} can be applied to evaluate how significant of the maximum periodogram coordinate and to obtain the corresponding dominant periodicity.
% % In terms of the statistical tests used for periodicity detection, two widely used tests are Fisher's test~\cite{fisher1929tests,wichert2004identifying} for dominant periodicity. Fisher's test is based on the Fourier periodogram, and has been successfully applied in various real-world signals. Specifically, the $g$-statistic in Fisher's test is introduced by using the maximum periodogram coordinate. 
% However, periodogram is not accurate when the period length is long or the time series is with sharp edges. 
% %In addition, it is not easy to determine the threshold for autocorrelation in the time domain. 
% %the power spectral density 
% %In periodogram-based methods, or spectral density based methods.
% %The periodogram-based methods can give a 
% % ACF-based approaches
% The ACF measures the similarity between a sequence and itself for some lags. Intuitively, a time series is periodic with a period length $T$ if it can be divided into equal segments with length $T$ sharing high similarities. In other words, the ACF whose lag is the multipliers of $T$ would be locally maximum or peaks. Based on the properties of ACF, numerous methods have been proposed, including the analysis of autocorrelation peaks~\cite{Wang2006}, autocorrelation zero-distance~\cite{Toller2019}. However, the estimation of ACF and the automated discovery of its maximum values can be affected by outliers and noises easily, which leads to many false alarms in practice.

% Combined approaches
Different periodicity detection algorithms have been proposed in data mining, signal processing, astrology, etc.
Periodicity detection can be performed in frequency domain~\cite{fisher1929tests,wichert2004identifying}, time domain~\cite{Wang2006,Toller2019}, or joint frequency-time domain~\cite{cPD_vlachos2005Autoperiod}. 
Frequency domain methods often rely on periodogram after Fourier transform. One widely used test based on periodogram is Fisher's test~\cite{fisher1929tests,wichert2004identifying} for dominant periodicity. Time domain methods often rely on ACF, which measures the similarity between a sequence and itself for some lags. 
% Intuitively, a time series is periodic with a period length $T$ if it can be divided into equal segments with length $T$ sharing high similarities. 
Besides, ensemble method~\cite{Toller2019} is also proposed recently to combine multiple periodicity detection methods together. 
% to combine the advantages of both methods. In AUTOPERIOD proposed in \cite{cPD_vlachos2005Autoperiod}, it first selects a list of candidates in the frequency domain using periodogram, and then identifies the exact period length in the time domain using ACF. The intuitive idea is that a valid period from the periodogram should lie on a hill of ACF. 
%  proposes an ensemble method which combines multiple periodicity detection methods together. Compared with AUTOPERIOD, it selects the list of candidate periods using both frequency domain methods and time domain methods. Also different properties of autocorrelation of periodic time series are utilized to validate period. Unfortunately, it is computationally expensive and its performance is also affected by outliers.
% Some other recent works on periodicity detection
Recently, some robust method like \cite{cPD_parthasarathy2006robust} is proposed by tracking the candidate periods using a Kalman filter. It achieves some robustness, but has limited resistance to severe noise and missing values. 
% This scheme tries to handle non-stationary time series using a sliding window, but its method is not universally applicable. 
In~\cite{dPD_li2012mining}, a method immune to noisy and incomplete observations is proposed, but it can only handle binary sequences.
% \cite{dPD_yuan2017detecting} also proposes a method to detect multiple periodicities, but it mainly focuses on discrete event sequences. 
In order to handle missing values in time series, the Lomb-Scargle periodograms~\cite{lomb1976least,scargle1982studies} is adopted to detect periodicity in \cite{glynn2006detecting,hu2014periodicity}. Unfortunately, the Lomb-Scargle periodogram does not perform well in periodicity detection of time series with non-Gaussian noise and non-sinusoidal shapes~\cite{schimmel2001emphasizing}. Some other types of periodicity detection algorithms include wavelet transform based method~\cite{Abdullah:testing:periodicity}, dynamic time warping based method~\cite{elfeky2005warp}, epoch folding~\cite{Graham2013}, etc. 
Unfortunately, existing methods cannot robustly deal with severe noise, trend changes,  outliers, and missing data simultaneously.






%The works in~\cite{glynn2006detecting,hu2014periodicity} adopt Lomb-Scargle periodograms~\cite{lomb1976least,scargle1982studies} to detect periodicity on datasets with missing data. Lomb-Scargle periodogram does not perform well in periodicity detection of time series with non-Gaussian noise and non-sinusoidal shapes



%periodicity detection in discrete time event ~\cite{dPD_li2012mining,ghosh2017finding,dPD_yuan2017detecting,otunba2014mbpd,rasheed2011efficient}


 
%(TODO) add a table to compare all algorithms.





% Statistical tests used in periodicity test


%  and Siegel's test~\cite{Siegel1980} for multiple periodicities. 
% The Siegel's test generalizes the Fisher's test by considering all large periodogram values to overcome the multiple peak problem when multiple periodicities occur. 


%Fisher proposed a test of hidden periodicities in a time series using the maximum periodogram coordinate by introducing the $g$-statistic~\cite{Aylmer1929}. The distribution of $g$-statistics can be computed exactly under a Gaussian process. Also note that large values of $g$ lead to the rejection of the null hypothesis. 





%%%%%%%%%%%%%% backup for intro and related work
%The detection of periodicity is the prerequisite of decomposition. In many real-world applications, it is required to detect multi-seasonalities and also be robust to abrupt trend changes and outliers.

 




% \begin{itemize}

% \item existing Periodicity Detection methods: continues TS Periodicity methods:

% Fisher's Test \cite{Aylmer1929} for single period;
% Siegel's Test for multiple periods \cite{Siegel1980}

% \cite{Toller2019, cPD_vlachos2005Autoperiod, elfeky2005warp, cPD_parthasarathy2006robust}

%   ={On periodicity detection and structural periodic similarity},

%   ={Robust periodicity detection algorithms},
  
%   ={{WARP}: time warping for periodicity detection}
  
  
  
  
  
  
  
  

% \item discrete TS PD methods, \cite{rasheed2011efficient, dPD_li2012mining,otunba2014mbpd, ghosh2017finding,dPD_yuan2017detecting}

%   ={Efficient periodicity mining in time series databases using suffix trees},
  
%   ={Mining event periodicity from incomplete observations},
  
%      ={{MBPD}: Motif-based period detection},
  
%      ={Finding Periodic Discrete Events in Noisy Streams},
    
%   ={Detecting Multiple Periods and Periodic Patterns in Event Time Sequences},
   
   
% \item recent wavelet in ICDM and KDD, \cite{zhao2018forecasting, wang2018multilevel}
   
%   ={Forecasting Wavelet Transformed Time Series with Attentive Neural Networks},
  
%   ={Multilevel wavelet decomposition network for interpretable time series analysis},
  
  
  
% \item wavelet review and book in data minning and ts, \cite{li2002survey, chaovalit2011discrete, rhif2019wavelet,addison2017illustrated, percival2006wavelet}
%   ={A survey on wavelet applications in data mining},
%   ={Discrete wavelet transform-based time series analysis and mining},
%   ={Wavelet Transform Application for/in Non-Stationary Time-Series Analysis: A Review},
%   =Wavelet methods for time series analysis
  
 
  
% \item MODWT(maximal overlap discrete wavelet transform, undecimated DWT)\cite{shensa1992discrete, nason1995stationary, nason1999wavelets}
  
%   ={The discrete wavelet transform: wedding the a trous and Mallat algorithms},
%   ={The stationary wavelet transform and some statistical applications},
%   ={Wavelets in time-series analysis}
  
% % \item wavelet entropy concept \cite{rosso2001wavelet} 
% %   ={Wavelet entropy: a new tool for analysis of short duration brain electrical signals},
  
% \item robust  Periodogram \cite{ACFPSD_kat98robustMperiodogram, li2008laplace}
%   ={Robust M-periodogram},
%   ={Laplace periodogram for time series analysis},


% \item Periodicity Detection for STL:  \cite{STL_cleveland1990stl,RobustSTL_wen2018robuststl, STR_dokumentov2015str,TBATS_de2011forecasting}
%  or trend filtering: \cite{hodrick1997postwar,kim2009ell_1}

%   ={{STL}: A Seasonal-Trend Decomposition Procedure Based on Loess},
%   ={RobustSTL: A Robust Seasonal-Trend Decomposition Algorithm for Long Time Series},
%   ={{STR}: A Seasonal-Trend Decomposition Procedure Based on Regression},
%   ={Forecasting Time Series with Complex Seasonal Patterns using Exponential Smoothing},
  
%   ={Postwar {US} business cycles: an empirical investigation},
%   ={$\ell_1$ Trend Filtering},
 
 
%  \item Periodicity Detection for Anomaly detection \cite{rasheed2013framework}, Forecasting~\cite{prema2015time, theodosiou2011forecasting}, search engine data mining ~\cite{vlachos2004identifying,drutsa2015engagement}
 
%  ={A framework for periodic outlier pattern detection in time-series sequences}
%  ={Time series decomposition model for accurate wind speed forecast}

% ={Identifying similarities, periodicities and bursts for online search queries}
%  ={Engagement periodicity in search engine usage: Analysis and its application to search quality evaluation}
%  ={Periodicity in user engagement with a search engine and its application to online controlled experiments}

 
% Daubechies wavelet family \cite{Daubechies1992}
% MODWT Wavelet for TS analysis \cite{percival2000wavelet,shensa1992discrete}
% O(N) for DWT \cite{Mallat1989}

 
% \end{itemize}
